Rollback-Free Stable Brick Structures Generation

While autoregressive models have advanced 3D generation, creating physically stable brick structures remains a challenge due to the strict requirements of gravity and interconnectivity. Existing approaches rely on external physical simulators during inference to perform rejection sampling and brick-by-brick rollbacks, which severely bottlenecks efficiency. To address this, we propose a reinforcement learning paradigm that shifts physical validity enforcement from test-time correction to training-time policy optimization. By utilizing assembly-level rewards, the model optimizes for collision avoidance, global connectivity, structural interlocking, and shape conformity. This paradigm allows the model to internalize physical priors, enabling the first rollback-free generation of stable brick structures. Experimental results demonstrate that our approach achieves state-of-the-art generation quality while accelerating inference speed by orders of magnitude. Our code and dataset are available at https://github.com/miniHuiHui/STABLE. Our models are available at https://huggingface.co/miniHui/STABLE.

==> _tab/ablation.tex <==
\begin{table*}[t]
\centering
\caption{
Reward ablation results. All variants are GRPO-trained from the same SFT initialization.
``w/o Connectivity'' removes $R_{\mathrm{conn}}$.
``w/o Structural'' removes both $R_{\mathrm{inter}}$ and $R_{\mathrm{conn}}$, leaving only collision and shape rewards.
``w/o Collision'' removes $R_{\mathrm{col}}$ while keeping shape, interlocking, and connectivity rewards.
}
\label{tab:reward_ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule
& \multicolumn{4}{c}{\textbf{Active Rewards}}
& \multicolumn{5}{c}{\textbf{Evaluation Metrics}} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-10}
\textbf{Variant}
& $R_{\mathrm{col}}$
& $R_{\mathrm{shape}}$
& $R_{\mathrm{inter}}$
& $R_{\mathrm{conn}}$
& \makecell{Coll.-Free\\Rate}
& \makecell{Voxel\\IoU}
& \makecell{Conn.\\Ratio}
& \makecell{Interlock.\\Score}
& \makecell{Composite\\Score} \\
\midrule
\textbf{\textsc{STABLE}}
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$
& \textbf{0.96} & 0.907 & \textbf{0.940} & 0.722 & \textbf{0.758} \\
w/o Connectivity
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $\times$
& 0.93 & 0.919 & 0.914 & 0.709 & 0.737 \\
w/o Structural
& $\checkmark$ & $\checkmark$ & $\times$ & $\times$
& \textbf{0.96} & \textbf{0.978} & 0.461 & 0.069 & 0.499 \\
w/o Collision
& $\times$ & $\checkmark$ & $\checkmark$ & $\checkmark$
& 0.92 & 0.897 & 0.910 & \textbf{0.734} & 0.737 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> _tab/ablation_details.tex <==
\begin{table}[t]
\centering
\caption{
Supplementary statistics on 100 test samples. ``Mean Coll. Voxels'' counts voxels occupied by more than one brick. ``Connected Rate'' measures the fraction of generations that form a single connected component. ``In-Bounds Rate'' measures the fraction of parseable generations whose bricks remain within the voxel world.
}
\label{tab:detailed_stats}
\begin{tabular}{lcccc}
\toprule
\textbf{Method}
& \makecell{Mean\\Bricks}
& \makecell{Mean Coll.\\Voxels}
& \makecell{Connected\\Rate}
& \makecell{In-Bounds\\Rate} \\
\midrule
Qwen3.5-2B 
& --- & --- & 0.00 & --- \\
BrickGPT
& 110.9 & 5.2 & 0.00 & 1.00 \\
SFT
& 661.5 & 585.8 & 0.00 & 0.79 \\
\textbf{\textsc{STABLE}}
& 216.5 & \textbf{0.05} & \textbf{0.49} & \textbf{1.00} \\
\midrule
w/o Connectivity
& 230.0 & 9.5 & 0.45 & 1.00 \\
w/o Structural
& 387.0 & 12.5 & 0.02 & 0.76 \\
w/o Collision
& 247.1 & 0.51 & 0.46 & 1.00 \\
\bottomrule
\end{tabular}
\end{table}

==> _tab/table_stage_effect.tex <==
\begin{table}[t]
\centering
\caption{Effect of supervised scaffolding and reward-based policy learning. SFT learns the point-cloud-to-brick format but does not produce collision-free structures, while \textsc{STABLE} substantially reduces voxel-level violations.}
\label{tab:stage_effect}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}
& \makecell{Parse\\Rate}
& \makecell{Voxel\\IoU}
& \makecell{Coll.-Free\\Rate}
& \makecell{Mean Coll.\\Voxels}
& \makecell{In-Bounds\\Rate}
& \makecell{Mean\\Bricks} \\
\midrule
Qwen3.5-2B Base
& 0.00 & 0.000 & 0.00 & 0.0 & 0.00 & 0.0 \\
SFT
& 0.97 & 0.813 & 0.00 & 585.8 & 0.79 & 661.5 \\
\textbf{\textsc{STABLE}}
& \textbf{1.00} & \textbf{0.907} & \textbf{0.96} & \textbf{0.05} & \textbf{1.00} & 216.5 \\
\bottomrule
\end{tabular}%
}
\end{table}

